A Survey of Resource-efficient LLM and Multimodal Foundation Models

Large foundation models, including large language models (LLMs), vision transformers (ViTs), diffusion, and LLM-based multimodal models, are revolutionizing the entire machine learning lifecycle, from training to deployment. However, the substantial advancements in versatility and performance these models offer come at a significant cost in terms of hardware resources. To support the growth of these large models in a scalable and environmentally sustainable way, there has been a considerable focus on developing resource-efficient strategies. This survey delves into the critical importance of such research, examining both algorithmic and systemic aspects. It offers a comprehensive analysis and valuable insights gleaned from existing literature, encompassing a broad array of topics from cutting-edge model architectures and training/serving algorithms to practical system designs and implementations. The goal of this survey is to provide an overarching understanding of how current approaches are tackling the resource challenges posed by large foundation models and to potentially inspire future breakthroughs in this field.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.
	       

==> fig-alg-compression-overview.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=black,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-red!10, text=black, align=left,font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]

\begin{figure*}[htpb]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\large,
                rectangle,
                draw=black,
                rounded corners,
                align=left,
                text centered,
                minimum width=4em,
                edge+={black, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=12em,font=\normalsize,}{},
            where level=2{text width=12em,font=\normalsize,}{},
            [
                \textbf{Model Compression}, ver
                        [
                          \textbf{Pruning}, fill=green!10
                          [
                          \textbf{Structured Pruning}, fill=green!10
                          [                          
                          LLM-Pruner~\cite{ma2023llm}{, }
                          LoRAPrune~\cite{zhang2023pruning}{,}
                          Sheared LLaMA~\cite{xia2023sheared}{,}
                          AdaPrune~\cite{hubara2021accelerated}{,}
                          GUM~\cite{santacroce2023matters}{,} \\
                          PLATON~\cite{zhang2022platon}{,}
                          SpAtten~\cite{wang2021spatten}{,}
                          DJPQ~\cite{wang2020differentiable}{,}
                          Block-Skim~\cite{guan2022block}{,}
                          DepGraph~\cite{fang2023depgraph}, 
                          leaf, text width=37.6em
                          ]
                          ]
                          [
                          \textbf{Unstructured Pruning}, fill=green!10
                          [
                          SparseGPT~\cite{frantar2023sparsegpt}{, }
                          Wanda~\cite{sun2023simple}{, }
                          Upop~\cite{shi2023upop}{, }
                          SIGE~\cite{li2022efficient},
                          leaf, text width=37.6em
                          ]
                          ]
                        ]
                        [
                          \textbf{Knowledge Distillation}, fill=green!10 
                          [
                          \textbf{Black-box KD}, fill=green!10
                          [
                            Meta-ICL~\cite{min2021metaicl}{, }
                            Metal-ICL~\cite{chen2021meta} {, }
                            Multitask-ICT~\cite{huang2022context}{, }
                            Lion~\cite{jiang2023lion}{, }
                            LaMini-LM~\cite{wu2023lamini} {, } \\
                            SSLM~\cite{fu2023specializing} {, }
                            Distilling Step-by-Step~\cite{hsieh2023distilling} {, }
                            Fine-tune-CoT~\cite{ho2022large}{, }
                            SOCRATIC CoT~\cite{shridhar2023distilling}{, } \\
                            DISCO~\cite{chen2023disco}{, } 
                            SCOTT~\cite{wang2023scott}{, }
                            SCoTD~\cite{li2023symbolic}{, }
                            MT-COT~\cite{li2022explanations} {, } \\
                            CoT Prompting~\cite{magister2022teaching}{, }
                            PaD~\cite{zhu2023pad},
                          leaf, text width=37.6em
                          ]
                          ]
                          [
                          \textbf{White-box KD}, fill=green!10
                          [
                            Baby Llama~\cite{timiryasov2023baby}{, }
                            MiniLLM~\cite{gu2023knowledge} {, }
                            GKD~\cite{agarwal2023gkd}{, }
                            KPTD~\cite{padmanabhan2023propagating}{, }
                            TED~\cite{liang2023less}{, } \\
                            MixKD~\cite{liang2020mixkd}{, }
                            DIME-FM~\cite{sun2023dime},
                          leaf, text width=37.6em
                          ]
                          ]
                        ] 
                        [
                          \textbf{Quantization}, fill=green!10 
                          [
                          \textbf{Quantization-Aware}\\\textbf{Training}, fill=green!10
                         [
                          LLM-QAT~\cite{liu2023llm}{, }
                          QuantGPT~\cite{tao2022compression}{,}
                          BitNet~\cite{wang2023bitnet},
                          leaf, text width=37.6em
                          ]
                          ]
                          [
                          \textbf{Post-Training}\\\textbf{Quantization}, fill=green!10
                          [
                          \textbf{Weight Quantization}, fill=green!10, text width=15em
                          [
                          LLM.int8()~\cite{dettmers2022llm}{, }
                          LUT-GEMM~\cite{park2023lut}{, }
                          OBQ~\cite{frantar2022optimal}{, } \\
                          Few-bit Backward~\cite{novikov2023few}{, } 
                          SqueezeLLM~\cite{kim2023squeezellm}{, }\\
                          SpQR~\cite{dettmers2023spqr}{, }
                          AWQ~\cite{lin2023awq}{, }
                          GPTQ~\cite{frantar2022gptq}{, }
                          QuIP~\cite{chee2023quip}{, } \\
                          OWQ~\cite{lee2023owq}{, } 
                          FineQuant~\cite{kim2023finequant},
                          leaf, text width=21em
                          ]
                          ]
                          [
                        \textbf{Weights-Activation}\\\textbf{Co-Quantization}, fill=green!10, text width=15em
                          [
                          BinaryBERT~\cite{novikov2023few}{, } 
                          I-BERT~\cite{bai2020binarybert}{, }
                          Q-ViT~\cite{li2022q}{, } \\
                          I-ViT~\cite{li2023vit}{, } 
                          OFQ~\cite{liu2023oscillation}{, } 
                          Q-Diffusion~\cite{li2023q}{, }  \\
                          Outlier Suppression~\cite{wei2022outlier}{, } \\
                          Outlier Suppression+~\cite{wei2023outlier}{, } 
                          ZeroQuant~\cite{yao2022zeroquant}{, } \\
                          ZeroQuant-V2~\cite{yao2023zeroquant}{, } 
                          ZeroQuant-FP~\cite{wu2023zeroquant}{, } \\ 
                          SmoothQuant~\cite{xiao2023smoothquant}{, } 
                          RPTQ~\cite{yuan2023rptq}{, } \\
                          OliVe~\cite{guo2023olive}{, } 
                          QLLM~\cite{liu2023qllm}{, } 
                          MoFQ~\cite{zhang2023integer}{, } \\
                          FlexRound~\cite{lee2023flexround}{,}
                          OmniQuant~\cite{shao2023omniquant},
                          leaf, text width=21em
                          ]
                          ]
                          ]
                        ] 
                        [
                          \textbf{Low-Rank Decomposition}, fill=green!10 
                          [
                            LoRD~\cite{kaushal2023lord}{, }
                            TensorGPT~\cite{xu2023tensorgpt}{, }
                            LoSparse~\cite{li2023losparse} {, }
                            ViTALiTy~\cite{dass2023vitality}{, }
                            ZeroQuant-V2~\cite{yao2023zeroquant},
                          leaf, text width=51.3em 
                          ]
                        ] 
                    ]
        \end{forest}
    }
    
    \caption{Overview of Model Compressions.}
    \label{fig:alg-compression-overview}
\end{figure*}

==> fig-algo-serving.tex <==
\begin{figure*}
	\centering
	\includegraphics[width=0.78\textwidth]{figs/fig-algo-serving.pdf}
%  \vspace{-10pt}	
	\caption{
		Serving algorithms and their roles in foundation model serving pipeline.
		}
	\label{fig:bkg-vit}
\end{figure*}

==> fig-bkg-llm-timeline.tex <==
\definecolor{cdqPurple}{RGB}{128,0,128}
\definecolor{cdqGrey}{gray}{0.7}
\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{figs/fig-bkg-llm-timeline.pdf}
 \vspace{-10pt}	
	\caption{
		Milestone model of LLM development, including: 
		\textcolor{blue!50}{Encoder-only}, 
		\textcolor{orange!50}{Decoder-only},
		\textcolor{red!50}{Encoder-Decoder}, 
		\textcolor{green!40}{Speech}, 
		\textcolor{cdqPurple}{MoE} and 
		\textcolor{cdqGrey}{Close-sourced LLM}.
		}
	\label{fig:bkg-llm-timeline}
\end{figure*}

==> fig-bkg-mm-arch.tex <==
\begin{figure*}
	\centering
	\includegraphics[width=0.68\textwidth]{figs/fig-bkg-mm-arch-modify.pdf}
%  \vspace{-10pt}	
	\caption{
		The architecture of multimodal models. 
		}
	\label{fig:bkg-mm-arch}
\end{figure*}

==> fig-bkg-models.tex <==
\begin{figure*}
	\centering
	\includegraphics[width=0.58\textwidth]{figs/fig-bkg-tree.pdf}
%  \vspace{-10pt}	
	\caption{
		The evolutionary tree of the milestone foundation models.
		}
	\label{fig:bkg-tree}
\end{figure*}

==> fig-bkg-transformer.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=0.7\textwidth]{figs/fig-bkg-transformer.pdf}
	\caption{Transformer Architecture~\cite{vaswani2017attention}. 
	% \cdq{put them into ppt and merge into one figure.}
	}
		\label{fig:bkg-transformer}
\end{figure}


==> fig-bkg-vit.tex <==
\begin{figure*}
	\centering
	\includegraphics[width=0.58\textwidth]{figs/fig-bkg-vit.pdf}
%  \vspace{-10pt}	
	\caption{
		Vision Transformer (ViT) architecture~\cite{dosovitskiy2020image}. 
		}
	\label{fig:bkg-vit}
\end{figure*}

==> fig-intro-AI-elec-v2.tex <==
\begin{figure*}
	\centering
	\includegraphics[width=0.85\textwidth]{figs/fig-intro-AI-elec-v2.pdf}
%  \vspace{-10pt}	
	\caption{
		Electricity Consumption: A Comparison between Countries and AI. 
		}
	\label{fig:intro-AI-elec}
\end{figure*}

==> fig-resource-efficient-famous-framework.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=black,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-red!10, text=black, align=left,font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]

\begin{figure*}[htpb]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\large,
                rectangle,
                draw=black,
                rounded corners,
                align=left,
                text centered,
                minimum width=4em,
                edge+={black, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=16em,font=\normalsize,}{},
            where level=2{text width=12em,font=\normalsize,}{},
            [
                \textbf{Resource-efficient Systems}, ver  
                        [
                            \textbf{Training}, fill=green!10
                            [
                            \textbf{Pre-training}, fill=green!10
                            [
                            ADA~\cite{ermis2022memory}{, }
                            MetaTroll~\cite{tian2023metatroll}{, }
                            ST-Adapter~\cite{pan2022st}{, }
                            HiWi~\cite{liao2023parameter}{, }\\
                            AdadMix~\cite{wang2022adamix}{, }
                            Residual Adapters~\cite{tomanek2021residual}{, }
                            PEMA~\cite{kim2023pema}, 
                            leaf, text width=25em
                            ]
                            ]
                            [
                            \textbf{Fine-tuning}, fill=green!10
                            [
                            ADA~\cite{ermis2022memory}{, }
                            MetaTroll~\cite{tian2023metatroll}{, }
                            ST-Adapter~\cite{pan2022st}{, }
                            HiWi~\cite{liao2023parameter}{, }\\
                            AdadMix~\cite{wang2022adamix}{, }
                            Residual Adapters~\cite{tomanek2021residual}{, }
                            PEMA~\cite{kim2023pema}, 
                            leaf, text width=25em
                            ]
                            ]
                            [
                            \textbf{Federated learning}, fill=green!10
                            [
                            ADA~\cite{ermis2022memory}{, }
                            MetaTroll~\cite{tian2023metatroll}{, }
                            ST-Adapter~\cite{pan2022st}{, }
                            HiWi~\cite{liao2023parameter}{, }\\
                            AdadMix~\cite{wang2022adamix}{, }
                            Residual Adapters~\cite{tomanek2021residual}{, }
                            PEMA~\cite{kim2023pema}, 
                            leaf, text width=25em
                            ]
                            ]
                        ]
                        [
                          \textbf{Serving}, fill=green!10
                          [
                            \textbf{Cloud}, fill=green!10
                            [
                            ADA~\cite{ermis2022memory}{, }
                            MetaTroll~\cite{tian2023metatroll}{, }
                            ST-Adapter~\cite{pan2022st}{, }
                            HiWi~\cite{liao2023parameter}{, }\\
                            AdadMix~\cite{wang2022adamix}{, }
                            Residual Adapters~\cite{tomanek2021residual}{, }
                            PEMA~\cite{kim2023pema}, 
                            leaf, text width=25em
                            ]
                          ]
                          [
                            \textbf{Edge}, fill=green!10
                            [
                            ADA~\cite{ermis2022memory}{, }
                            MetaTroll~\cite{tian2023metatroll}{, }
                            ST-Adapter~\cite{pan2022st}{, }
                            HiWi~\cite{liao2023parameter}{, }\\
                            AdadMix~\cite{wang2022adamix}{, }
                            Residual Adapters~\cite{tomanek2021residual}{, }
                            PEMA~\cite{kim2023pema}, 
                            leaf, text width=25em
                            ]
                          ]
                        ]
                    ]
        \end{forest}
    }
    
    \caption{Summary of famous resource-efficient open-source frameworks.}
    \label{fig:tree-resource-efficient-framework-tree}
\end{figure*}

==> fig-resource-efficient-finetuning-algorithm.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=black,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-red!10, text=black, align=left,font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]

\begin{figure*}[htpb]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\large,
                rectangle,
                draw=black,
                rounded corners,
                align=left,
                text centered,
                minimum width=4em,
                edge+={black, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=16em,font=\normalsize,}{},
            where level=2{text width=12em,font=\normalsize,}{},
            [
                \textbf{Fine-tuning Algorithms}, ver  
                        [
                            \textbf{Additive}, fill=green!10
                            [
                            \textbf{Adapter}, fill=green!10
                            [
                            ADA~\cite{ermis2022memory}{, }
                            MetaTroll~\cite{tian2023metatroll}{, }
                            ST-Adapter~\cite{pan2022st}{, }
                            HiWi~\cite{liao2023parameter}{, }\\
                            AdadMix~\cite{wang2022adamix}{, }
                            Residual Adapters~\cite{tomanek2021residual}{, }
                            PEMA~\cite{kim2023pema}, 
                            leaf, text width=25em
                            ]
                            ]
                            [
                            \textbf{Prompt}, fill=green!10
                            [
                            PromptTuning ~\cite{lester2021power}{, }
                            ATTEMPT~\cite{asai2022attempt}{, }
                            BioInstruct ~\cite{tran2023bioinstruct}{, }\\
                            DualPL ~\cite{yang2023dual}{, }
                            MPrompt ~\cite{chen2023mprompt}{, }
                            DPT ~\cite{xiao2023decomposed}, 
                            leaf, text width=25em
                            ]
                            ]
                            [
                            \textbf{Prefix}, fill=green!10
                            [
                            UAPT ~\cite{wang2023user}{, }
                            Prefix-diffusion ~\cite{liu2023prefix}{, }
                            DOP ~\cite{zhao2022domain}{, }
                            DAPA ~\cite{nair2023domain}{, }\\
                            PIP ~\cite{wan2023pip}{, }
                            Prefix Propagation ~\cite{li2023prefix}{, } 
                            APT ~\cite{zhang2023towards},
                            leaf, text width=25em
                            ]
                            ]
                        ]
                        [
                          \textbf{Selective}, fill=green!10
                          [
                            SAM~\cite{fu2023effectiveness}{, }
                            Token Mixing~\cite{liu2023token}{, }
                            VL-PET~\cite{hu2023vl}{, }
                            SPT~\cite{he2023sensitivity}{, }
                            SmartFRZ~\cite{li2022smartfrz}{, }
                            FiSH-DiP~\cite{das2023unified},
                          leaf, 
                          text width=38.7em
                          ]
                        ]
                        [
                          \textbf{Re-parameter}, fill=green!10 
                          [
                            EfficientDM~\cite{he2023efficientdm}{, }
                            LoftQ~\cite{li2023loftq}{, }
                            PEQA~\cite{kim2023memory}{, }
                            QLoRA~\cite{dettmers2023qlora}{, }
                            GLoRA~\cite{chavan2023one}{, }
                            LongLoRA~\cite{chen2023longlora}{, }\\
                            PELA~\cite{guo2023learning}{, }
                            LBP-WHT~\cite{yang2023efficient}{, }
                            DSEE~\cite{chen2021dsee}{, }
                            Dynamic-Pooling~\cite{nawrot2022efficient},
                          leaf, text width=38.7em
                          ]
                        ] 
                    ]
        \end{forest}
    }
    
    \caption{Summary of resource-efficient fine-tuning algorithms.}
    \label{fig:tree-resource-efficient-fintuning-algorithms-tree}
\end{figure*}

==> fig-resource-efficient-inference-algo.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=black,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-red!10, text=black, align=left,font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]

\begin{figure*}[htpb]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\large,
                rectangle,
                draw=black,
                rounded corners,
                align=left,
                text centered,
                minimum width=4em,
                edge+={black, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=16em,font=\normalsize,}{},
            where level=2{text width=12em,font=\normalsize,}{},
            where level=3{text width=12em,font=\normalsize,}{},
            [
                \textbf{Inference Algorithms}, ver  
                [
                    \textbf{Opportunistic Decoding}, fill=green!10
                    [
                        \textbf{Speculative Decoding}, fill=green!10
                        [
                        Yaniv Leviathan et al.~\cite{Leviathan2022FastIF}{, }
                        SpecTr~\cite{sun2023spectr}{, }
                        ProphetNet~\cite{Yan2020ProphetNetPF}{, } \\
                        Draft \& Verify~\cite{Zhang2023DraftV}{, }
                        Medusa~\cite{medusa}{, }
                        Look ahead decoding~\cite{fu2023lookahead}{, } \\
                        SpecInfer~\cite{miao2023specinfer}{, }
                        LLMCad~\cite{xu2023llmcad}{, }
                        Speculative Sampling~\cite{Chen2023AcceleratingLL},
                        leaf, text width=28em
                        ]
                    ]
                    [
                        \textbf{Look up Decoding}, fill=green!10
                        [
                        Prompt cache~\cite{gim2023prompt}{, }
                        LLMA~\cite{yang2023inference},
                        leaf, text width=15em
                        ]
                    ]
                    [
                        Skeleton-of-Thought~\cite{ning2023skeletonofthought},
                        leaf, text width=12em
                    ]
                ]
                [
                    \textbf{Input Filtering/Compression}, fill=green!10
                    [
                        \textbf{Prompt Compression}, fill=green!10
                        [
                        LLMLingua~\cite{jiang2023llmlingua}{, }
                        Huiqiang Jiang et al.~\cite{wingate2022prompt}{, }
                        EntropyRank~\cite{tsvetkov2023entropyrank}{, } \\
                        AutoCompressors~\cite{chevalier2023adapting}{, }
                        ICAE~\cite{ge2023incontext}{, }
                        Nugget 2D~\cite{qin2023nugget}{, }
                        CoT-Max~\cite{huang2023boosting},
                        leaf, text width=31em
                        ]
                    ]
                    [
                        \textbf{Token Pruning}, fill=green!10
                        [
                        SpAtten~\cite{wang2021spatten}{, }
                        PuMer~\cite{cao2023pumer}{, }
                        Dynamic Context Pruning~\cite{anagnostidis2023dynamic}{, }
                        HVT~\cite{pan2021scalable}{, }\\
                        DynamicViT~\cite{rao2021dynamicvit}{, }
                        Liang et al.~\cite{liang2022patches}{, }
                        AdaViT~\cite{meng2021adavit}{, }
                        A-ViT~\cite{yin2022adavit}{, }\\
                        ATS~\cite{fayyaz2022adaptive}{, }
                        Evo-ViT~\cite{xu2021evovit}{, }
                        SPViT~\cite{kong2022spvit}{, }
                        PoWER-BERT~\cite{goyal2020powerbert}{, }\\
                        Length-Adaptive Transformer~\cite{kim2021lengthadaptive}{, }
                        TR-BERT~\cite{ye2021trbert}{, }
                        LTP~\cite{kim2022learned},
                        leaf, text width=31em
                        ]
                    ]
                ]
                [
                    \textbf{KV Cache Optimizations}, fill=green!10
                    [
                        \textbf{Activation Quantization}, fill=green!10
                        [
                        ATOM~\cite{zhao2023atom}{, }
                        LLM.int8()~\cite{dettmers2022llm}{, }
                        OmniQuant~\cite{shao2023omniquant}{, }
                        ZeroQuant-FP~\cite{wu2023zeroquantfp}{, }\\
                        Outlier Suppression~\cite{wei2023outlier}{, }
                        QLLM~\cite{liu2023qllm}{, }
                        OliVe~\cite{guo2023olive}{, }
                        RPTQ~\cite{yuan2023rptq}{, }\\
                        LLM-FP4~\cite{liu2023llmfp4}{, }
                        SmoothQuant~\cite{xiao2023smoothquant},
                        leaf, text width=31em
                        ]
                    ]
                    [
                        \textbf{Memory Efficient}\\ 
                        \textbf{Sparse Attention}, fill=green!10
                        [
                        Landmark Attention~\cite{mohtashami2023landmark}{,}
                        H2O~\cite{zhang2023h2o}{, }\\
                        Dynamic Context Pruning~\cite{anagnostidis2023dynamic}{, }
                        Scissorhands~\cite{liu2023scissorhands},
                        leaf, text width=22em
                        ]
                    ]
                    [
                        \textbf{Block-wise Managing}, fill=green!10
                        [
                        vLLM~\cite{vllm},
                        leaf, text width=5em
                        ]
                    ]
                ]
                [
                    \textbf{Long Context/Super Resolution}\\
                    \textbf{Oriented Optimizations}, fill=green!10
                    [
                        \textbf{Prerequisite:}\\ \textbf{Positional Encoding}, fill=green!10
                        [
                        ALiBi~\cite{press2021train}{,}
                        xPOS~\cite{sun2022length}{,}
                        CLEX~\cite{chen2023clex}{,}
                        Linear Interpolation~\cite{chen2023extending}{,}
                        \\NTK Interpolation~\cite{SketchyRedditPost2023}{,}
                        YaRN Interpolation~\cite{peng2023yarn}{,}
                        FIRE~\cite{DBLP:journals/corr/abs-2310-04418}{,}
                        PoSE~\cite{zhu2023pose}
                        , leaf, text width=32em
                        ]
                    ]
                    [
                        \textbf{Resource-efficient}\\ 
                        \textbf{optimizations}, fill=green!10
                        [
                            \textbf{Recurrent Structure}, fill=green!10
                            [
                            Transformer-XL~\cite{dai2019transformer}{,}
                            Memformer~\cite{wu2020memformer}{,}\\
                            % $\infty$-former~\cite{martins2021infty}{,}
                            RMT~\cite{bulatov2022recurrent}{,}\\
                            Block-Recurrent Transformer~\cite{hutchins2022block}
                            % \yws{moving it to architecture section is better?}
                            , leaf, text width=17em 
                            ]
                        ]
                        % [
                            % \textbf{Memory-Retrieval}\\ 
                            % \textbf{Augmentation}, fill=green!10
                            % [
                            % KNN-augmented Transformer~\cite{wu2022memorizing}{,}\\
                            % LongMem~\cite{wang2023augmenting}{,}\\
                            % Unlimiformer~\cite{bertsch2023unlimiformer}{,}\\
                            % Focused Transformer~\cite{tworkowski2023focused}{,}\\
                            % Xu et al.~\cite{Xu2023RetrievalML}, 
                            % leaf, text width=19em 
                            % ]
                        % ]
                        [
                            \textbf{Attention Optimizations}, fill=green!10
                            [
                            Landmark Attention~\cite{mohtashami2023landmark}{, }\\
                            LM-Infinite~\cite{han2023lminfinite}{, }
                            StreamingLLM~\cite{xiao2023efficient}{,}\\
                            PCW~\cite{ratner2023parallel}{,}
                            LongNet~\cite{ding2023longnet}{,}
                            SLED~\cite{ivgi2023efficient}
                            , leaf, text width=17em 
                            ]
                        ]
                    ]
                ]
            ]
        \end{forest}
    }
    \caption{Summary of resource-efficient inference algorithms.}
    \label{fig:tree-resource-efficient-inference-tree}
\end{figure*}

==> fig-tree-federated-fine-tuning-systems.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=black,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-red!10, text=black, align=left,font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]

\begin{figure*}[htpb]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\large,
                rectangle,
                draw=black,
                rounded corners,
                align=left,
                text centered,
                minimum width=4em,
                edge+={black, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=16em,font=\normalsize,}{},
            where level=2{text width=12em,font=\normalsize,}{},
            [
                \textbf{Federated Fine-tuning}, ver
                        
                    ]
        \end{forest}
    }
    
    \caption{Summary of resource-efficient federated fine-tuning systems.}
    \label{fig:tree-resource-efficient federated fine-tuning systems tree}
\end{figure*}

==> sec-architecture-multimodal.tex <==
\subsection{Multimodal Variants}




==> sec-diffusion-bkgnd.tex <==
\subsection{Diffusion Model}\label{subsec:diffusion-model}

Diffusion models in image generation use a noise reduction process to create high-quality images by evicting the redundant noise in the image. In the training stage, these models introduce noise into an image, transforming it into a random state. In the inference stage, this process is reversed, with the noise being progressively removed. This denoising process is essential for improving image clarity, leading to images with high resolution and detailed sharpness.

Stable diffusion models have taken this technology a step further. They are uniquely capable of generating images that are not only of high quality but also tailored to specific textual descriptions. This fusion of text and image generation opens up new avenues for creating images that accurately reflect given text prompts, broadening the scope of their application.

The subsequent section will delve into the fundamental structure of the diffusion model, encompassing U-Net, VAE image encoder-decoder, and CLIP text encoder. Additionally, downstream tasks associated with the diffusion model will be explored, followed by an cost analysis of the diffusion model. Table~\ref{tab:bkgd-diffusion} summarizes the typical diffusion models/methods and their typical tasks.

\input{tab-bkgd-diffusion}

\subsubsection{Key Architecture}

\begin{figure*}
    \centering
    \includegraphics[width=0.6\textwidth]{figs/fig-sd-arch.png}
    \caption{Stable diffusion architecture~\cite{rombach2022high}}
    \label{fig:bkg-sd-arch}
\end{figure*}

Diffusion models incorporate three key components: an image encoder/decoder, a denoising network, and a text encoder. Each plays a crucial role in the model's ability to generate detailed and contextually relevant images. Figure~\ref{fig:bkg-sd-arch} shows the architecture of the stable diffusion model. The model mainly consists of three parts: image encoder/decoder, denoising network, and text encoder.

\textbf{Image Encoder/Decoder}. This part of the diffusion model is responsible for processing images. The encoder takes an input image and compresses it into a lower-dimensional latent representation. This compression is crucial for reducing the computational load and making the model more efficient. The decoder then works in reverse, taking the latent representation and reconstructing it back into a high-resolution image. This process is essential for the model's ability to generate detailed visual content. 
In diffusion models, VAE is often employed as the image encoder/decoder. The VAE~\cite{kingma2013auto} model is a generative model that is employed to learn the latent space of the image. The VAE model consists of an encoder and a decoder. The encoder is responsible for mapping the image to the latent space, while the decoder is responsible for mapping the latent space to the image space. Both encoder and decoder network are often built with convolutional neural layers. The VAE model is trained by minimizing the reconstruction loss and the KL divergence loss. The reconstruction loss is responsible for ensuring that the image generated by the decoder is similar to the original image, while the KL divergence loss is responsible for ensuring that the latent space is similar to the standard normal distribution. The VAE model is employed in the diffusion model to learn the latent space of the image. 
Another variant of VAE model that is often employed in the diffusion tasks is VQ-VAE~\cite{van2017neural}, to learn the latent space of the image through a vector quantization layer. The vector quantization layer applies vector quantization technique, quantizing each pixel of the image to the nearest codebook vector. In this way, VQ-VAE model can encode and decode the image in a more efficient way.

\textbf{Denoising Network}. Denoising network progressively removes noise from the encoded images. Initially, during the training phase, the model adds noise to the images, gradually leading them to a state of pure randomness. The denoising network then learns to reverse this noise addition, step by step, during the inference phase. This gradual denoising is crucial for enhancing the clarity and quality of the final image output. U-Net is often employed as the denoising network in diffusion models. The U-Net~\cite{ronneberger2015u} model is a convolutional neural network model that is employed for noise prediction. Figure~\ref{fig:bkg-unet} shows the architecture of the U-Net model. Each blue box in the schematic represents a multi-channel feature map, with the number of channels annotated above the box. Dimensions on the x-y plane are indicated at the box's lower left corner. Feature maps that are replicated are depicted as white boxes. The various procedural operations within the framework are denoted by arrows, illustrating the flow and interaction of the feature maps.
The U-Net is a fully convolutional network that consists of a contracting path and an expansive path. The contracting path is responsible for capturing context information in the image by mapping the image to high dimension space, while the expansive path facilitates precise localization by upsampling. To retain the information of the contracting path, the expansive path is connected to the contracting path via skip connections. The U-Net model is a popular choice for image segmentation tasks, and is also employed in the diffusion model to predict noise within an image.
    

\textbf{Text Encoder}. The text encoder is a vital component for text-to-image generation tasks. It processes textual descriptions and converts them into a format that the model can understand and utilize. This component allows the stable diffusion model to generate images that are not just high in quality but also accurately reflect the content described in the text inputs. The text encoder enables the model to bridge the gap between textual descriptions and visual content, making it possible to create images that are contextually aligned with the provided text. There are various text encoders that are employed in the diffusion model, such as CLIP~\cite{radford2021learning} in stable diffusion. CLIP is an innovative model that intertwines the understanding of visual and textual data, which is employed in stable diffusion for text-controlled image generation. It comprises two main components, a Vision Transformer and a Text Transformer, and jointly learns an image encoder and a text encoder to predict the correct pairings of a batch of (image, text).
The Vision Transformer processes images with a series of convolutional layers to convert an input image into a sequence of flattened 2D patches. These patches are then linearly embedded and processed through multiple self-attention layers. The self-attention layers allow the model to weigh different parts of the image differently, focusing on the most relevant parts for understanding the image in the context of a given text.
In parallel, the Text Transformer is responsible for processing natural language input. It uses a similar Transformer architecture, but instead of image patches, it processes word embeddings. The Transformer layers in this block employ self-attention mechanisms to understand the context and relationships between words in a sentence, enabling the model to grasp the nuances of language.
The key innovation of CLIP lies in its ability to project the outputs of both the Vision and Text Transformers into a joint shared embedding space, allowing the model to perform tasks like matching images with appropriate text descriptions or vice versa.

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.6\textwidth]{figs/fig-clip-arch.pdf}
%     \caption{CLIP methodology~\cite{radford2021learning}. \mwx{not needed?}}
%     \label{fig:bkg-clip}
% \end{figure*}




\subsubsection{Foundation Models and Downstream Tasks}

In the domain of image generation with diffusion models, numerous foundational models are available, each capable of being applied to a variety of downstream tasks. These models have been designed to handle tasks ranging from generating high-quality images to performing image inpainting, editing, and super-resolution. Their design allows for adaptability across different applications in image processing and generation.

\textbf{Stable Diffusion}. Stable diffusion~\cite{rombach2022high} is a type of diffusion model known for its efficiency and effectiveness in generating high-quality images. It operates by gradually refining noise in images through a learned process, leading to clear and detailed visual outputs. This model is particularly versatile, finding applications in various downstream tasks such as generating detailed images from text descriptions (text-to-image generation), restoring or completing parts of images (image inpainting), modifying specific aspects of existing images (image editing), and enhancing the resolution of images (image super-resolution). Stable diffusion's adaptability in these areas makes it a valuable tool in the field of image processing and generation.

\textbf{Consistency models}. Consistency models~\cite{song2023consistency} are generative models developed to enhance the efficiency of diffusion models in generating high-quality images, audio, and video. They enable fast single-step generation, overcoming the slow sampling speed of traditional diffusion models. These models are capable of zero-shot data editing tasks like image inpainting, colorization, and super-resolution, without requiring specific training for these tasks. They can be trained by distilling pre-trained diffusion models or as standalone models.

\textbf{DALL-E}. DALL-E~\cite{ramesh2021zero} is primarily used for image generation, capable of creating diverse, complex images from textual descriptions. This model combines aspects of natural language understanding and computer vision, enabling it to generate images that accurately reflect a wide range of textual prompts, from simple descriptions to elaborate scenarios. DALL-E's applications extend to various downstream tasks, including creating unique artwork and illustrations, designing product prototypes, generating visual content for advertising and social media, and aiding in educational materials by visualizing concepts and ideas. Its versatility in translating textual inputs into visual outputs makes it a powerful tool for creative, educational, and commercial endeavors.


\textbf{DreamBooth}. DreamBooth~\cite{ruiz2023dreambooth} is a specialized generative model that personalizes text-to-image diffusion models to specific subjects or objects while retaining their original generative capabilities. It achieves this by fine-tuning a pre-trained diffusion model on a small set of images featuring the target subject. DreamBooth can be applied to various downstream tasks such as creating personalized avatars or characters, generating images of specific objects or people in different contexts, and customizing artwork or design elements to include particular subjects. Its ability to tailor the generative process to individual subjects makes it particularly useful in applications requiring a high degree of personalization or specificity in image generation.


\begin{comment}
\textbf{Image Generation}. Diffusion models in image generation showcase dual capabilities, i.e., randomly generating images learned from the training data, and also creating images guided by textual descriptions. In random generation~\cite{ho2020denoising, nichol2021improved, song2020denoising, zhang2022gddim}, they produce a wide range of images, from realistic to artistic, by refining noise into structured visuals. In text-to-image generation~\cite{rombach2022high, nichol2021glide, ho2022cascaded, batzolis2021conditional, hu2022global}, they interpret and visualize written descriptions, accurately transforming text into corresponding images. 
LDM~\cite{rombach2022high} efficiently generate high-quality images in a compressed latent space under textual guidance, balancing reduced computational load with rapid. GLIDE~\cite{nichol2021glide} produces photorealistic samples using classifier-free guidance of diffusion model. Cascaded Diffusion~\cite{ho2022cascaded} generates high-resolution images with a cascaded diffusion model, which is a pipeline of multiple diffusion models that generate images of increasing resolution.
This blend of random and text-driven creation highlights their versatility, making them powerful tools for content creation, art, and design.

\textbf{Image Inpainting}. Image inpainting~\cite{lugmayr2022repaint, zhang2023towards, yang2023uni, corneanu2024latentpaint} with diffusion models involves filling in missing or damaged parts of images. 
RePaint~\cite{lugmayr2022repaint} produces high-quality and diverse output images for any inpainting form, which s applicable to even extreme masks.
Uni-paint~\cite{yang2023uni} is a versatile framework for multimodal inpainting that supports various guidance modes such as unconditional, text, stroke, exemplar-driven, and their combinations for diverse image restoration needs.
These models effectively understand the context and content around the missing areas and generate plausible fill-ins that seamlessly blend with the original image. This is especially valuable in photo restoration and editing tasks.

\textbf{Image Editing}. In image ~\cite{kawar2023imagic, zhang2023sine, pan2023effective, couairon2022diffedit}, diffusion models allow for precise modifications of existing images. Whether it's changing specific features like color and texture or altering entire scenes, these models can adaptively adjust images while maintaining a natural and coherent overall appearance. For instance, Imagic~\cite{kawar2023imagic} is a novel method enabling complex, text-guided semantic edits on single real images, such as altering object postures or compositions, by utilizing a pre-trained text-to-image diffusion model for precise alignment and fine-tuning to preserve image characteristics. 
SINE~\cite{zhang2023sine} is an innovative approach for single-image editing using diffusion models, offering a novel model-based guidance and patch-based fine-tuning to enable content creation and editing on individual images while addressing overfitting and maintaining content integrity.

\textbf{Image Super-Resolution}. For image super-resolution~\cite{li2022srdiff, yue2023resshift, wu2023hsr}, diffusion models are used to enhance the resolution and clarity of low-resolution images. They achieve this by adding finer details and reducing artifacts, effectively 'upscaling' the image quality. For example, SRDiff~\cite{li2022srdiff} is the first diffusion-based model for single image super-resolution, designed to generate diverse, high-quality super-resolution images from low-resolution inputs, offering advantages in detail, training efficiency, and flexible image manipulation. ResShift~\cite{Resshift} is an innovative diffusion-based super-resolution model that significantly reduces diffusion steps for faster inference, using a Markov chain to efficiently transition between high and low-resolution images, achieving superior or comparable performance to existing methods with minimal sampling steps.
This application is particularly beneficial in improving the quality of old or low-quality images in media, medical imaging, and surveillance.

\end{comment}


\begin{comment}
\textbf{Training algorithm.}
A DDPM~\cite{ho2020denoising} utilizes two Markov chains: the forward chain, which distorts data into noise, typically aiming for a standard Gaussian distribution, and the reverse chain, which reconstructs the original data from this noise. 
The core idea of the DDPM forward process is gradually adding noise to an image over a series of steps, transforming it into a random noise distribution. In each step, a small amount of Gaussian noise is added to the data, making the image slightly more noisy. This process is repeated many times, resulting in an image that is entirely random noise.
DDPM learns to reverse the diffusion process. The model is trained to remove the noise added in the diffusion process. Essentially, it learns to predict the noise that was added at each step and then subtracts this noise, restoring the image to its previous state. This denoising process is iteratively applied, starting from pure noise and gradually reconstructing the original image.

Formally, given the training data $x_0$ following the distribution $q(x_0)$, the time step $t$ and noise $\epsilon$ are sampled respectively from a uniform distribution $Uniform(\{1\dots\mathbf{T}\})$ and a Gaussian distribution $\mathbf{N}(\mathbf{0}, \mathbf{I})$. The noise is add to the training data according to Eq.\ref{eq:ddpm-add-noise}, where $\bar\alpha_t$ is a constant hyperparameter. The training target is to minimize the mean square error between predicted noise and the original noise added to the data, i.e., the diffusion model takes gradient descent step on Eq.\ref{eq:ddpm-grad-descent}, where $\epsilon_\theta$ denotes the noise prediction network that takes noised data and time step as input and predict the added noise.

\begin{align}
    \sqrt{\bar\alpha_t} x_0 + \sqrt{1-\bar\alpha_t}\epsilon \label{eq:ddpm-add-noise}
\end{align}
\begin{align}
    \nabla_\theta \left\| \epsilon - \epsilon_\theta(\sqrt{\bar\alpha_t} x_0 + \sqrt{1-\bar\alpha_t}\epsilon, t) \right\|^2 \label{eq:ddpm-grad-descent}
\end{align}

\textbf{Sampling algorithm.}
After the noise is predicted, the diffusion model can remove the predicted noise from the noised image through sampling algorithm. Formally, given a sample $x-t$ at time step $t$, the model can get the sample $x_{t-1}$ according to Eq.\ref{eq:ddpm-sampling}, where $\alpha_t$ is a constant hyperparameter. The process of predicting noise and sampling is repeated $\mathbf{T}$ times until the noise is completely eliminated, resulting in $x_0$.

\begin{align}
    &x_{t-1} = \frac{1}{\sqrt{\alpha_t}}\left( x_t - \frac{1-\alpha_t}{\sqrt{1-\bar\alpha_t}} \epsilon_\theta(x_t, t) \right) + \sigma_t z \label{eq:ddpm-sampling}
    \\
    &where\ \ z \sim \mathbf{N}(\mathbf{0}, \mathbf{I})\quad if\ t > 1,\ else\ z\ =\ \mathbf{0}. \notag
\end{align}
\end{comment}



\subsubsection{Cost Analysis}

\begin{figure*}
    \centering
    \includegraphics[width=0.85\textwidth]{figs/fig-sd2-1-cost.pdf}
    \caption{Parameters and FLOPs percentage of Stable Diffusion 2.1.}
    \label{fig:bkg-diffusion-cost}
\end{figure*}

In this section, we will examine the cost associated with each critical component of the diffusion model. Given the variable sizes of these modules in diffusion models, our analysis will focus on Stable Diffusion 2.1 as a representative example for this discussion. Stable Diffusion 2.1 incorporates a U-Net for denoising, a VAE for image encoding and decoding, and a CLIP model as the text encdoer. Figure~\ref{fig:bkg-diffusion-cost}(a) and (e) shows the FLOPs and parameter number percentage in the stable diffusion 2.1 model. Figure~\ref{fig:bkg-diffusion-cost}(b) and (f) shows the FLOPs and parameter number percentage in the VAE model. Figure~\ref{fig:bkg-diffusion-cost}(c) and (g) shows the FLOPs and parameter number percentage in the U-Net model. Figure~\ref{fig:bkg-diffusion-cost}(d) and (h) shows the FLOPs and parameter number percentage in the CLIP model.

\textbf{U-Net}. The U-Net of Stable Diffusion 2.1 takes image latents of shape 4$\times$96$\times$96 as input and predicts noise in the latent space. The model is trained on the LAION-5B dataset~\cite{schuhmann2022laion}. The U-Net has 865M parameters, with total FLOPs of 759G for processing a sample.

\textbf{VAE} Stable Diffusion 2.1 incorporates a VAE that encodes images to latent space and decode them. The VAE takes images with resolution 3$\times$768$\times$768 as input and encode them to 4$\times$96$\times$96. The VAE is co-trained with the U-Net on the same dataset. The VAE has 83M parameters, with total FLOPs of 4T for processing a sample.

\textbf{CLIP}. Stable Diffusion 2.1 uses the CLIP~\cite{radford2021learning} model for text encoding. The CLIP model is trained on various (image, text) pair dataset, such as LAION dataset and DataComp dataset~\cite{gadre2023datacomp}. The CLIP model takes sentence as the input and encodes each token to hidden vector with size 1024. The model has 289M parameters, with total FLOPs of 289M for processing a signle token. 




==> sec-systems-device.tex <==
\subsection{On-device Inference Systems}
\begin{itemize}
    \item edge-cloud co-design
    \item MOE
    \item Memory optimization
    \item Kernel optimization
\end{itemize}

==> sec-systems-general.tex <==
\subsection{General-purpose Optimizations}
\begin{itemize}
    \item Cache optimization
    \item Fusion optimization
\end{itemize}
For both cloud and edge 

kernel and graph optimization.

==> tab-bkgd-diffusion.tex <==
\begin{sidewaystable}[]

    \centering
    \footnotesize
    \caption{Typical diffusion models/methods and their typical tasks.}
    \label{tab:bkgd-diffusion}
    \begin{tabular}{|l|l|l|l|l|l|}
        \hline
        Model Name       & Killer Tasks                                                            & Pre-training Method                                                   & Pre-training Datasets                                                                      & Testing Datasets                                                                                                      & Testing Metrics                                                              \\ \hline
        UNet             & image segmentation                                                      & supervisied                                                           & Carvana                                                                                    & Carvana                                                                                                               & precision, recall, F1                                                        \\ \hline
        VAVAE            & \begin{tabular}[c]{@{}l@{}}image encoding\\ image decoding\end{tabular} & unsupervised                                                          & CIFAR10, ImageNet, VCTK                                                                    & /                                                                                                                     & /                                                                            \\ \hline
        DDPM             & image generation                                                        & unsupervised                                                          & \begin{tabular}[c]{@{}l@{}}CIFAR, ImageNet, \\ CelebA, LSUN\end{tabular}                   & \begin{tabular}[c]{@{}l@{}}CIFAR, ImageNet, \\ CelebA, LSUN\end{tabular}                                              & FID                                                                          \\ \hline
        Improved DDPM    & image generation                                                        & unsupervised                                                          & \begin{tabular}[c]{@{}l@{}}CIFAR, ImageNet, \\ CelebA, LSUN\end{tabular}                   & \begin{tabular}[c]{@{}l@{}}CIFAR, ImageNet, \\ CelebA, LSUN\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}log-likelihood, \\ precision, recall\end{tabular} \\ \hline
        DDIM             & image generation                                                        & unsupervised                                                          & \begin{tabular}[c]{@{}l@{}}CIFAR, ImageNet, \\ CelebA, LSUN\end{tabular}                   & \begin{tabular}[c]{@{}l@{}}CIFAR, ImageNet, \\ CelebA, LSUN\end{tabular}                                              & FID                                                                          \\ \hline
        gDDIM            & image generation                                                        & unsupervised                                                          & \begin{tabular}[c]{@{}l@{}}CIFAR, ImageNet, \\ CelebA, LSUN\end{tabular}                   & \begin{tabular}[c]{@{}l@{}}CIFAR, ImageNet, \\ CelebA, LSUN\end{tabular}                                              & FID                                                                          \\ \hline
        CLIP             & image generation                                                        & self-supervised                                                       & publicly image-caption data                                                                & \begin{tabular}[c]{@{}l@{}}ImageNet, CIFAR-10, \\ CIFAR-100, MNIST, \\ STL-10, Oxford-IIIT Pet, Food-101\end{tabular} & accuracy                                                                     \\ \hline
        Stable Diffusion & image generation                                                        & unsupervised                                                          & \begin{tabular}[c]{@{}l@{}}CIFAR, ImageNet, \\ CelebA, LSUN\end{tabular}                   & \begin{tabular}[c]{@{}l@{}}CIFAR, ImageNet, \\ CelebA, LSUN\end{tabular}                                              & FID                                                                          \\ \hline
        VQ-Diffusion     & image generation                                                        & supervisied                                                           & \begin{tabular}[c]{@{}l@{}}CUB-200, Oxford-102, \\ MSCOCO, FFHQ, and ImageNet\end{tabular} & \begin{tabular}[c]{@{}l@{}}CUB-200, Oxford-102, \\ MSCOCO, FFHQ, ImageNet\end{tabular}                                & FID                                                                          \\ \hline
        SnapFusion       & image generation                                                        & unsupervised                                                          & MS-COCO                                                                                    & MS-COCO                                                                                                               & FID                                                                          \\ \hline
        ScaleCrafter     & image generation                                                        & /                                                                     & \begin{tabular}[c]{@{}l@{}}CIFAR, ImageNet, \\ CelebA, LSUN\end{tabular}                   & \begin{tabular}[c]{@{}l@{}}CIFAR, ImageNet, \\ CelebA, LSUN\end{tabular}                                              & FID                                                                          \\ \hline
        FreeU            & image generation                                                        & no-training                                                           & /                                                                                          & /                                                                                                                     & FID                                                                          \\ \hline
        PNDM             & image generation                                                        & unsupervised                                                          & Cifar10, CelebA, LSUN                                                                      & Cifar10, CelebA, LSUN                                                                                                 & FID                                                                          \\ \hline
        DPM-solver       & image generation                                                        & unsupervised                                                          & CIFAR-10, CelebA, ImageNet                                                                 & CIFAR-10, CelebA, ImageNet                                                                                            & FID                                                                          \\ \hline
        ResShift         & super resulution                                                        & unsupervised                                                          & ImageNet                                                                                   & ImageNet                                                                                                              & /                                                                            \\ \hline
        SRDDiff          & super resulution                                                        & /                                                                     & CelebA and DIV2K                                                                           & CelebA and DIV2K                                                                                                      & PSNR, SSIM, LPIPS                                                            \\ \hline
        RePaing          & Image Inpainting                                                        & /                                                                     & \begin{tabular}[c]{@{}l@{}}Cifar10, LSUN-church, \\ LSUN-bedroom, CelebA\end{tabular}      & \begin{tabular}[c]{@{}l@{}}Cifar10, LSUN-church, \\ LSUN-bedroom, CelebA\end{tabular}                                 & user study                                                                   \\ \hline
        Uni-paint        & Image Inpainting                                                        & /                                                                     & \begin{tabular}[c]{@{}l@{}}EditBench, Unsplash website, \\ synthetical images\end{tabular} & \begin{tabular}[c]{@{}l@{}}EditBench, Unsplash website, \\ synthetical images\end{tabular}                            & NIMA, RMSE                                                                   \\ \hline
        Imagic           & Image Editing                                                           & \begin{tabular}[c]{@{}l@{}}supervised and\\ unsupervised\end{tabular} & /                                                                                          & /                                                                                                                     & User study                                                                   \\ \hline
        SINE             & Image Editing                                                           & /                                                                     & LAION                                                                                      & LAION                                                                                                                 & /                                                                            \\ \hline
        \end{tabular}
\end{sidewaystable}
